Unsupervised Search Algorithm Configuration using Query Performance Prediction

Search engine configuration can be quite difficult for inexpert developers. Instead, an auto-configuration approach can be used to speed up development time. Yet, such an automatic process usually requires relevance labels to train a supervised model. In this work, we suggest a simple solution based on query performance prediction that requires no relevance labels but only a sample of queries in a given domain. Using two example usecases we demonstrate the merits of our solution.

==> abstract.tex <==
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER PLACEHOLDER 
